Mask-Induced Displacement in Audio XAI via Logit Trajectory Decomposition

Perturbation-based XAI methods for audio classifiers often estimate feature importance by masking spectrogram regions and crediting output changes to the retained signal. Yet they typically assume the fill (the mask replacement) is negligible. We propose logit-space trajectory decomposition to examine this assumption. An on-axis component captures output along a line connecting the fully filled (occluded) spectrogram to the fully retained original; an off-axis component captures perpendicular displacement. We evaluate across three fills, three audio classifiers, and 1,100 AudioSet clips. We demonstrate that no fill is acoustically neutral under full occlusion: Zero fill activates silence and Gaussian Noise fill activates broadband noise. Under partial masking, 41-77% of output displacement is off-axis, with the direction of the residual stable across mask retention fraction and specific to each model-fill combination. Attribution methods are unevenly exposed to off-axis displacement through their sampling and weighting strategies, revealing apparatus-dependence. Where the off-axis residual is stable and low-dimensional, its structure affords mitigation.

==> assets/foc_gauss_cls.tex <==
\fontsize{8}{10}\selectfont
\definecolor{crimson}{HTML}{D7263D}
\definecolor{tigerflame}{HTML}{C4933F}
\definecolor{spaceindigo}{HTML}{D7263D}
\definecolor{verdigris}{HTML}{1A7A4A}
\caption{Modal top-1 class and mean sigmoid $\bar{q}$ per source class under \fillgauss fill at full occlusion. Label colour and marker indicate semantic group: $^\P${\color{tigerflame}broadband noise} (White noise, Static, Silence), $^\dagger${\color{verdigris}electrical interference} (Hum); uncoloured labels fall outside these groups.\looseness=-1}
\vspace{0.5em}
\label{tab:foc_gauss_cls}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabularx}{\linewidth}{@{} >{\raggedright\arraybackslash}p{1.4cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X @{}}
\hline
 & \textbf{\astsa} & \textbf{\pannsns} & \textbf{\pannssa} \\
\hline
Frying food & \textcolor{tigerflame}{White noise}$^\P$ -- .50 & \textcolor{tigerflame}{White noise}$^\P$ -- .32 & \textcolor{tigerflame}{Static}$^\P$ -- .23 \\
Drum kit    & \textcolor{tigerflame}{White noise}$^\P$ -- .44 & \textcolor{tigerflame}{White noise}$^\P$ -- .32 & \textcolor{tigerflame}{Static}$^\P$ -- .17 \\
Owl         & \textcolor{tigerflame}{White noise}$^\P$ -- .37 & \textcolor{tigerflame}{White noise}$^\P$ -- .18 & \textcolor{tigerflame}{White noise}$^\P$ -- .10 \\
Heartbeat   & \textcolor{tigerflame}{White noise}$^\P$ -- .22 & \textcolor{tigerflame}{Silence}$^\P$ -- .19 & Music -- .17 \\
Whispering  & \textcolor{tigerflame}{White noise}$^\P$ -- .37 & \textcolor{tigerflame}{Static}$^\P$ -- .28 & Music -- .19 \\
Bagpipes    & \textcolor{tigerflame}{White noise}$^\P$ -- .25 & \textcolor{verdigris}{Hum}$^\dagger$ -- .10 & \textcolor{verdigris}{Hum}$^\dagger$ -- .14 \\
\hline
\end{tabularx}


==> assets/perturbation_algorithm.tex <==
\begin{algorithm}[h!]
\caption{Spectrogram Perturbation Pipeline}
\label{alg:perturbation}
\textbf{Input:} waveform $x$, model $\mathcal{F}$, fill matrix $\mathbf{Z}_{\text{fill}} \in \mathbb{C}^{F \times T}$, seeds $R$, samples per seed $L$ \\
\textbf{Output:} $\mathbf{m}_{r,l} \in \{0,1\}^{F \times T}$ (binary mask), $\mathbf{q}_{r,l} \in [0,1]^{527}$ (sigmoid confidence)
\begin{algorithmic}
\STATE Compute $\mathbf{S} = \Psi(\mathbf{Z}) \in \mathbb{R}^{M \times T}$
\STATE Define $M \times X$ cell grid; map $X \to T$
\STATE Compute $\mathbf{Z}_{\text{fill}}$ once per clip
\FOR{$r = 1$ \TO $R$}
    \STATE Randomly partition into $K_F \times K_T = K$ blocks
    \FOR{$l = 1$ \TO $L$}
        \STATE Sample $\mathbf{b} \in \{0,1\}^{K}$, each block $\sim \mathrm{Bernoulli}(0.5)$
        \STATE Expand $\mathbf{b}$ to $\mathbf{m}_{r,l} \in \{0,1\}^{F \times T}$ via filterbank mapping
        \STATE $\tilde{\mathbf{Z}} \leftarrow \mathbf{m}_{r,l} \odot \mathbf{Z} + (1 - \mathbf{m}_{r,l}) \odot \mathbf{Z}_{\text{fill}}$
        \STATE $\mathbf{q}_{r,l} \leftarrow \mathcal{F}(\Psi(\tilde{\mathbf{Z}}))$
    \ENDFOR
\ENDFOR
\RETURN $\{\mathbf{m}_{r,l}\}$, $\{\mathbf{q}_{r,l}\}$
\end{algorithmic}
\end{algorithm}

